SwinIA: Self-Supervised Blind-Spot Image Denoising without Convolutions

Self-supervised image denoising implies restoring the signal from a noisy image without access to the ground truth. State-of-the-art solutions for this task rely on predicting masked pixels with a fully-convolutional neural network. This most often requires multiple forward passes, information about the noise model, or intricate regularization functions. In this paper, we propose a Swin Transformer-based Image Autoencoder (SwinIA), the first fully-transformer architecture for self-supervised denoising. The flexibility of the attention mechanism helps to fulfill the blind-spot property that convolutional counterparts normally approximate. SwinIA can be trained end-to-end with a simple mean squared error loss without masking and does not require any prior knowledge about clean data or noise distribution. Simple to use, SwinIA establishes the state of the art on several common benchmarks.

==> paper/table/grayscale_vert.tex <==
\begin{table}[t!]
\small
  \centering
  \caption{Grayscale image denoising results for BSD68 and Set12 with synthetic noise along with the method description (supervision type and number of train and test passes). The highest PSNR(dB)/SSIM among self-supervised denoising methods is highlighted in \textbf{bold}, the second-best is \underline{underlined}. \textsuperscript{$\dag$} denotes the models that we implemented and trained ourselves.}
  \begin{tabular}[b]{cllcccc}
    \toprule
      & & Method & Train & Test & BSD68 & Set12 \\
    \midrule
      \multirow{8}{*}[-1.7ex]{\rotatebox{90}{\shortstack[c]{Gaussian $\sigma=15$ \\ \hphantom{0} \\ \hphantom{0}}}} 
        & \multirow{2}{*}{\textit{Supervised}} & N2C & 1 & 1 & 31.58/0.889 & 32.60/0.899 \\
        && SwinIR & 1 & 1 & 31.97/\hphantom{0}---\hphantom{.0} & 33.36/\hphantom{0}---\hphantom{.0} \\
      \cmidrule{2-7}
        & \multirow{4}{*}{\textit{Self-Supervised}} & R2R & 1 & 50 & \underline{31.54}/\textbf{0.885} & \textbf{32.54}/\textbf{0.897}  \\
        && Noise2Self\textsuperscript{$\dag$} & 1 & 1 & 30.63/0.843 & 29.88/0.840 \\
        && Noise2Same\textsuperscript{$\dag$} & 2 & 1 & 30.85/0.850 & 30.02/0.849 \\
        && Blind2Unblind & 17 & 1 & 31.44/0.884 & \underline{32.46}/\textbf{0.897}  \\
      \cmidrule{2-7}
        & \multirow{2}{*}{\shortstack[c]{\textit{Self-Supervised} \\ \textit{(BSN)}}} & Laine19 & 4 & 4 & --- & --- \\
        && Ours\textsuperscript{$\dag$} & 1 & 1 & \textbf{31.84}/\textbf{0.885} & 31.04/0.882 \\
    \midrule
      \multirow{8}{*}[-1.7ex]{\rotatebox{90}{\shortstack[c]{Gaussian $\sigma=25$ \\ \hphantom{0} \\ \hphantom{0}}}} 
        & \multirow{2}{*}{\textit{Supervised}} & N2C & 1 & 1 & 29.02/0.822 & 30.07/0.852 \\
        && SwinIR & 1 & 1 & 29.50/\hphantom{0}---\hphantom{.0} & 31.01/\hphantom{0}---\hphantom{.0} \\
      \cmidrule{2-7} 
        & \multirow{4}{*}{\textit{Self-Supervised}} & R2R & 1 & 50 & 28.99/0.818 & \underline{30.06}/\underline{0.851} \\
        && Noise2Self\textsuperscript{$\dag$} & 1 & 1 & 28.88/0.789 & 28.37  0.799 \\
        && Noise2Same\textsuperscript{$\dag$} & 2 & 1 & \underline{29.13}/0.800 & 28.54/0.814 \\
        && Blind2Unblind & 17 & 1 & 28.99/\underline{0.820} & \textbf{30.09/0.854}  \\
      \cmidrule{2-7}
        & \multirow{2}{*}{\shortstack[c]{\textit{Self-Supervised} \\ \textit{(BSN)}}} & Laine19 & 4 & 4 & 28.84/0.814 & --- \\
        && Ours\textsuperscript{$\dag$} & 1 & 1 & \textbf{30.01}/\textbf{0.837} & 29.61/0.848 \\
    \midrule
      \multirow{8}{*}[-1.7ex]{\rotatebox{90}{\shortstack[c]{Gaussian $\sigma=50$ \\ \hphantom{0} \\ \hphantom{0}}}} 
        & \multirow{2}{*}{\textit{Supervised}} & N2C & 1 & 1 & 26.08/0.715 & 26.88/0.777 \\
        && SwinIR & 1 & 1 & 26.58/\hphantom{0}---\hphantom{.0} & 27.91/\hphantom{0}---\hphantom{.0} \\
      \cmidrule{2-7} 
        & \multirow{4}{*}{\textit{Self-Supervised}} & R2R & 1 & 50 & 26.02/0.705 & {26.86}/{0.771} \\
        && Noise2Self\textsuperscript{$\dag$} & 1 & 1 & 26.19/0.664 & 25.56/0.692 \\
        && Noise2Same\textsuperscript{$\dag$} & 2 & 1 & \underline{26.75}/0.714 & 26.13/0.744 \\
        && Blind2Unblind & 17 & 1 & 26.09/\underline{0.715} & \textbf{26.91}/\textbf{0.776} \\
      \cmidrule{2-7}
        & \multirow{2}{*}{\shortstack[c]{\textit{Self-Supervised} \\ \textit{(BSN)}}} & Laine19 & 4 & 4 & 25.78/0.698 & --- \\
        && Ours\textsuperscript{$\dag$} & 1 & 1 & \textbf{27.23}/\textbf{0.743} & \underline{26.88}/\underline{0.772} \\
    \bottomrule
  \end{tabular}
  \label{tab:gray}
\end{table}

==> paper/table/synthetic_gaussian.tex <==
\begin{table}[ht!] % !htbp
\small
  \centering
  \caption{Denoising results on synthetic sRGB datasets with Gaussian synthetic noise along with the method description (supervision type and number of train and test passes). The highest PSNR(dB)/SSIM among self-supervised denoising methods is highlighted in \textbf{bold}, the second-best is \underline{underlined}. \textsuperscript{$\dag$}~denotes the models that we implemented and trained ourselves.}
  \begin{tabular}{cclccccc}
    \toprule
      && Method & train & test & KODAK & BSD300 & SET14 \\
    \midrule
      \multirow{16}{*}[-1.7ex]{\rotatebox{90}{\shortstack[c]{Gaussian $\sigma = 25$ \\ \hphantom{0} \\ \hphantom{0}}}} & \textit{Traditional} & CBM3D & - & - & 31.87/0.868 & 30.48/0.861 & 30.88/0.854 \\ 
    \cmidrule{2-8}
      &\multirow{2}{*}{\textit{Supervised}} & Noise2Clean & 1 & 1 & 32.43/0.884 & 31.05/0.879 & 31.40/0.869 \\
      && Noise2Noise & 1 & 1 & 32.41/0.884 & 31.04/0.878 & 31.37/0.868 \\
    \cmidrule{2-8}
      &\multirow{3}{*}{\shortstack[c]{\textit{Self-Supervised} \\ \textit{+ noise model}}} &Laine19-pme & 4 & 4 & 32.40/0.883 & 30.99/0.877 & 31.36/0.866 \\
      &&Honzatko-pme & 1 & 1 & 32.45/\hphantom{0}---\hphantom{.0} & 31.02/\hphantom{0}---\hphantom{.0} & 31.25/\hphantom{0}---\hphantom{.0} \\
      &&Noisier2Noise & 1 & 1 & 30.70/0.845 & 29.32/0.833 & 29.64/0.832 \\
    \cmidrule{2-8}
      &\multirow{6}{*}{\textit{Self-Supervised}} &Self2Self & 1 & 50 & 31.28/0.864 & 29.86/0.849 & 30.08/0.839 \\
      &&Noise2Void & 1 & 1 & 30.32/0.821 & 29.34/0.824 & 28.84/0.802 \\
      &&Noise2Same\textsuperscript{$\dag$} & 2 & 1 & 30.77/0.841 & 29.50/0.834 & 29.53/0.827 \\   
      &&DBSN & 2 & 1 & 31.64/0.856 & 29.80/0.839 & 30.63/0.846 \\
      &&R2R & 1 & 50 & 32.25/\underline{0.880} & \underline{30.91}/0.872 & \textbf{31.32}/\textbf{0.865} \\
      &&NBR2NBR & 2 & 1 & 32.08/0.879 & 30.79/\underline{0.873} & 31.09/\underline{0.864} \\  
      % && IDR & ? & ? & 32.36/0.884 & 31.48/0.890  & - \\
      &&B2UB & 17 & 1 & \textbf{32.27}/\underline{0.880} & 30.87/0.872 & 31.27/\underline{0.864} \\
      &&DCD-Net & 3 & 1 & \textbf{32.27}/\textbf{0.881} & \textbf{31.01}/\textbf{0.876} & \underline{31.29}/0.862 \\
    \cmidrule{2-8}
      &\multirow{2}{*}{\shortstack[c]{\textit{Self-Supervised} \\ \textit{(BSN)}}} & Laine19 & 4 & 4 & 30.62/0.840 & 28.62/0.803 & 29.93/0.830 \\
      &&Ours\textsuperscript{$\dag$} & 1 & 1 & 31.43/0.863 & 29.94/0.853 & 30.56/0.856 \\
    \midrule
      \multirow{15}{*}[-1.7ex]{\rotatebox{90}{\shortstack[c]{Gaussian $\sigma \in \left[5, 50\right]$ \\ \hphantom{0} \\ \hphantom{0}}}} &\textit{Traditional} & CBM3D & - & - & 32.02/0.860 & 30.56/0.847 & 30.94/0.849 \\ 
    \cmidrule{2-8}
      &\multirow{2}{*}{\textit{Supervised}} & Noise2Clean & 1 & 1 & 32.51/0.875 & 31.07/0.866 & 31.41/0.863 \\
      && Noise2Noise & 1 & 1 & 32.50/0.875 & 31.07/0.866 & 31.39/0.863 \\
    \cmidrule{2-8}
      &\multirow{2}{*}{\shortstack[c]{\textit{Self-Supervised} \\ \textit{+ noise model}}} &Laine19-pme & 4 & 4 & 32.40/0.870 & 30.95/0.861 & 31.21/0.855 \\
      &&Honzatko-pme & 1 & 1 & 32.46/\hphantom{0}---\hphantom{.0} & 31.18/\hphantom{0}---\hphantom{.0} & 31.25/\hphantom{0}---\hphantom{.0} \\
    \cmidrule{2-8}
      &\multirow{6}{*}{\textit{Self-Supervised}} &Self2Self & 1 & 50 & 31.37/0.860 & 29.87/0.841 & 29.97/0.849 \\
      &&Noise2Void & 1 & 1 & 30.44/0.806 & 29.31/0.801 & 29.01/0.792 \\
      &&Noise2Same\textsuperscript{$\dag$} & 2 & 1 & 30.78/0.835 & 29.49/0.823 & 29.34/0.817 \\   
      &&DBSN & 2 & 1 & 30.38/0.826 & 28.34/0.788 & 29.49/0.814 \\
      &&R2R & 1 & 50 & 31.50/0.850 & 30.56/0.855 & 30.84/0.850 \\
      &&NBR2NBR & 2 & 1 & 32.10/0.870 & 30.73/\underline{0.861} & 31.05/\textbf{0.858} \\  
      &&B2UB & 17 & 1 & \underline{32.34}/\textbf{0.872} & \underline{30.86}/\underline{0.861} & \textbf{31.14}/\underline{0.857} \\
      &&DCD-Net & 3 & 1 & \textbf{32.35}/\textbf{0.872} & \textbf{31.09}/\textbf{0.866} & \underline{31.09}/0.855 \\
    \cmidrule{2-8}
      &\multirow{2}{*}{\shortstack[c]{\textit{Self-Supervised} \\ \textit{(BSN)}}} & Laine19 & 4 & 4 & 30.52/0.833 & 28.43/0.794 & 29.71/0.822 \\
      &&Ours\textsuperscript{$\dag$} & 1 & 1 & 31.54/0.859 & 30.00/0.847 & 30.55/0.849 \\
    \bottomrule
  \end{tabular}
  \label{tab:sRGB-gauss}
\end{table}

==> paper/table/synthetic_poisson.tex <==
\begin{table}[ht!] % !htbp
\small
  \centering
  \caption{Denoising results on synthetic sRGB datasets with Poisson synthetic noise along with the method description (supervision type and number of train and test passes). The highest PSNR(dB)/SSIM among self-supervised denoising methods is highlighted in \textbf{bold}, the second-best is \underline{underlined}. \textsuperscript{$\dag$}~denotes the models that we implemented and trained ourselves.}
  \begin{tabular}{cclccccc}
    \toprule
      && Method & train & test & KODAK & BSD300 & SET14 \\
    \midrule
      \multirow{16}{*}[-1.7ex]{\rotatebox{90}{\shortstack[c]{Poisson $\lambda = 30$ \\ \hphantom{0} \\ \hphantom{0}}}} & \textit{Traditional} & Anscombe & - & - & 30.53/0.856 & 29.18/0.842 & 29.44/0.837 \\ 
    \cmidrule{2-8}
      &\multirow{2}{*}{\textit{Supervised}} & Noise2Clean & 1 & 1 & 31.78/0.876 & 30.36/0.868 & 30.57/0.858 \\ 
      &&Noise2Noise & 1 & 1  & 31.77/0.876 & 30.35/0.868 & 30.56/0.857 \\
    \cmidrule{2-8}
      &\multirow{2}{*}{\shortstack[c]{\textit{Self-sup.} \\ \textit{+ noise model}}} &Laine19-pme & 4 & 4 & 31.67/0.874 & 30.25/0.866 & 30.47/0.855 \\
      &&Honzatko-pme & 1 & 1 & 31.67/\hphantom{0}---\hphantom{.0}  & 30.25/\hphantom{0}---\hphantom{.0} & 30.14/\hphantom{0}---\hphantom{.0} \\
    \cmidrule{2-8}
      &\multirow{6}{*}{\textit{Self-sup.}} &Self2Self &  1 & 50  & 30.31/0.857 & 28.93/0.840 & 28.84/0.839 \\
      &&Noise2Void & 1 & 1  & 28.90/0.788 & 28.46/0.798 & 27.73/0.774 \\
      &&Noise2Same\textsuperscript{$\dag$} & 2 & 1 & 27.73/0.747 & 26.69/0.714 & 26.78/0.735 \\    
      &&DBSN & 2 & 1  & 30.07/0.827 & 28.19/0.790 & 29.16/0.814 \\
      &&R2R & 1 & 50 & 30.50/0.801 & 29.47/0.811 & 29.53/0.801 \\
      &&NBR2NBR & 2 & 1 & 31.44/0.870 & 30.10/\underline{0.863} & 30.29/\underline{0.853} \\
      &&B2UB & 17 & 1 & \underline{31.64}/\underline{0.871} & \underline{30.25}/0.862 & \underline{30.46}/0.852 \\ 
      && DCD-Net & 3 & 1 & \textbf{32.35}/\textbf{0.872} & \textbf{31.09}/\textbf{0.866} & \textbf{31.09}/\textbf{0.855} \\
    \cmidrule{2-8}
      &\multirow{2}{*}{\shortstack[c]{\textit{Self-sup.} \\ \textit{(true BSN)}}} &Laine19 & 4 & 4 & 30.19/0.833 & 28.25/0.794 & 29.35/0.820 \\
      &&Ours\textsuperscript{$\dag$} & 1 & 1 & 31.01/0.857 & 29.61/0.847 & 29.98/0.847 \\ 
    \midrule
      \multirow{16}{*}[-1.7ex]{\rotatebox{90}{\shortstack[c]{Poisson $\lambda \in \left[5, 50\right]$ \\ \hphantom{0} \\ \hphantom{0}}}} & \textit{Traditional} & Anscombe & - & - & 29.40/0.836 & 28.22/0.815 & 28.51/0.817 \\ 
    \cmidrule{2-8}
      &\multirow{2}{*}{\textit{Supervised}} & Noise2Clean & 1 & 1 & 31.19/0.861 & 29.79/0.848 & 30.02/0.842 \\ 
      &&Noise2Noise & 1 & 1 & 31.18/0.861 & 29.78/0.848 & 30.02/0.842 \\
    \cmidrule{2-8}
      &\multirow{2}{*}{\shortstack[c]{\textit{Self-sup.} \\ \textit{+ noise model}}} &Laine19-pme & 4 & 4 & 30.88/0.850 & 29.57/0.841 & 28.65/0.785 \\
      &&Honzatko-pme & 1 & 1 & --- & --- & ---\\
    \cmidrule{2-8}
      &\multirow{6}{*}{\textit{Self-sup.}} &Self2Self &  1 & 50  & 29.06/0.834 & 28.15/0.817 & 28.83/0.841 \\
      &&Noise2Void & 1 & 1 & 28.78/0.758 & 27.92/0.766 & 27.43/0.745 \\
      &&Noise2Same\textsuperscript{$\dag$} & 2 & 1 & 27.44/0.738 & 26.36/0.700 & 26.37/0.721 \\    
      &&DBSN & 2 & 1 & 29.60/0.811 & 27.81/0.771 & 28.72/0.800 \\
      &&R2R & 1 & 50 & 29.14/0.732 & 28.68/0.771 & 28.77/0.765 \\
      &&NBR2NBR & 2 & 1 & 30.86/0.855 & 29.54/0.843 & 29.79/0.838 \\
      &&B2UB & 17 & 1 & \textbf{31.07}/\textbf{0.857} & \underline{29.92}/\underline{0.852} & \textbf{30.10}/\textbf{0.844} \\ 
      && DCD-Net & 3 & 1 & \underline{31.00}/\textbf{0.857} & \textbf{29.99}/\textbf{0.855} & \underline{29.99}/\underline{0.843} \\
    \cmidrule{2-8}
      &\multirow{2}{*}{\shortstack[c]{\textit{Self-sup.} \\ \textit{(true BSN)}}} &Laine19 & 4 & 4 & 29.76/0.820 & 27.89/0.778 & 28.94/0.808 \\
      &&Ours\textsuperscript{$\dag$} & 1 & 1 & 30.29/0.835 & 28.84/0.818 & 29.35/0.827 \\  
    \bottomrule
  \end{tabular}
  \label{tab:sRGB-poiss}
\end{table}
